Construction Grammar Provides Unique Insight into Neural Language Models

Construction Grammar (CxG) has recently been used as the basis for probing studies that have investigated the performance of large pretrained language models (PLMs) with respect to the structure and meaning of constructions. In this position paper, we make suggestions for the continuation and augmentation of this line of research. We look at probing methodology that was not designed with CxG in mind, as well as probing methodology that was designed for specific constructions. We analyse selected previous work in detail, and provide our view of the most important challenges and research questions that this promising new field faces.

==> extras.tex <==
A core assumption of generative grammar \citep{chomsky1988}, which can be already found in Bloomfieldian structural linguistics 
\citep{Bloomfield.1933}, is a strict separation 
of lexicon and grammar: grammar is conceptualized as a set
of compositional and general rules that operate on a list
of arbitrary and specific lexical items in generating
syntactically well-formed sentences. This dichotomous view
was increasingly questioned in the 1980s when several
studies drew attention to the fact that linguistic units
larger than lexical items (e.g., idioms) can also possess
non-compositional meanings \citep{Langacker.1987,
Lakoff.1987, Fillmore.1988, Fillmore.1989}.
For instance, it is not clear how the effect of the words ``let alone'' (as in ``she doesn't eat fish,
let alone meat'') on both the syntax and the semantics of the rest of the sentence could be inferred from general syntactic rules \citep{Fillmore.1988}.
This insight about the ubiquity of stored form-meaning
pairings in language is
adopted as the central tenet
%elevated to the centerpiece
of
grammatical theory by Construction Grammar (CxG;
see \citet{hoffmann2013oxford} for a comprehensive
overview). Rather than a system divided into non-overlapping
syntactic rules and lexical items, CxG views language as a
structured system of constructions with varying
granularities that encapsulate syntactic and semantic
components as single linguistic signs---ranging from
individual morphemes up to phrasal elements and fixed
expressions \citep{Kay.1999, Goldberg.1995}. In this
framework, syntactic rules can be seen as emergent
abstractions over similar stored
constructions \citep{goldberg2003, Goldberg.2006}. A
different set of stored constructions can result in
different abstractions and thus different syntactic rules,
which allows CxG to naturally accommodate for the dynamic
nature of grammar as evidenced, for instance, by
inter-speaker variability and linguistic
change \citep{Hilpert.2006}.


